From the CDC to emerging infectious disease publics: The long-now of polarizing and complex health crises

This study examines how public discourse around COVID-19 unfolded on Twitter through the lens of crisis communication and digital publics. Analyzing over 275,000 tweets involving the CDC, we identify 16 distinct discourse clusters shaped by framing, sentiment, credibility, and network dynamics. We find that CDC messaging became a flashpoint for affective and ideological polarization, with users aligning along competing frames of science vs. freedom, and public health vs. political overreach. Most clusters formed echo chambers, while a few enabled cross cutting dialogue. Publics emerged not only around ideology but also around topical and emotional stakes, reflecting shifting concerns across different stages of the pandemic. While marginalized communities raised consistent equity concerns, these narratives struggled to reshape broader discourse. Our findings highlight the importance of long-term, adaptive engagement with diverse publics and propose design interventions such as multi-agent AI assistants, to support more inclusive communication throughout extended public health crises.

==> findings3.tex <==
\section{Study III: Findings}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        Topic & Breakpoint & p-value \\ \hline
        Masking and Vaccines & 2020-12-11 & **** \\ \hline
        Masking and Vaccines & 2021-07-27 & **** \\ \hline
        Spreading COVID-19 and Masks & 2020-11-14 & **** \\ \hline
        Masking in Schools & 2020-05-16 & **** \\ \hline
        Masking in Schools & 2020-05-16 & *** \\ \hline
    \end{tabular}
    \caption{Significant breakpoints}
    \label{tab:breakdown}
\end{table}

==> findings_2.tex <==
\section{Study I: Platform signals and message properties}
We start this section by analyzing how CDC discourse is affected by Twitter platform affordances (e.g., retweets, likes, etc.) in \S\ref{sec:finding_rt}. Next, we analyze how credibility of sources in a Twitter message, the use of rich media, and the sentiment of that message affect COVID discourse in the CDC public in \S\ref{sec:sent_photo_credibility}. Finally, in \S\ref{sec:verified_accts}, we analyze how user properties, like being verified or influential in the network (based on FFR), are associated with user behavior in the CDC public.

\paragraph{Summary of findings:} Discussions about vaccines are more likely to receive all kinds of Twitter engagement. Although positive tweets discussed the seriousness of COVID-19, they also shared news about dropping infection levels, especially after the lockdowns. Neutral accounts were more likely to discuss the lack of clarity in the CDC guidelines but avoided talking about mortality rates or engagement in political discourse–both features predictive of negative Tweets. We found that verified accounts, while less likely to Tweet, are more likely to be retweeted (thus the high echo score in Table \ref{tab:behavior_echo}), liked, receive responses, but not quote-tweets, and to use rich media. Tweets using low-credibility sources are also more likely to use rich media and be posted by verified accounts. The more frequently an account uses low-credibility sources, the more likely they are to mention other users.  

\begin{table}[h!]
    \centering
    \caption{This table compares the CDC, responses to it, verified users, and responses to them, tweets using pictures and responses to them, as well as the use of low-credibility sources and responses to these tweets. Specifically, we focus on the echo and average sentiment for each. Echo is the ratio between retweet/tweets. The closer the value to 1, the less the likelihood of their tweets being retweeted. The higher the echo the higher the number of retweets per Tweet. At times, the properties might overlap. For example, we show how often verified users use images.}
    \begin{tabular}{|p{2.5cm}|l|l|l|l|p{1cm}|l|l|}
    \hline
        \textbf{Behavior and Affordances} & \textbf{Total} & \textbf{Unique} & \textbf{Echo} & \textbf{Sent.} & \textbf{Low-cred. (\%)} & \textbf{Rich (\%)} & \textbf{Ver. (\%)} \\ \hline
        \textbf{CDC} & 2,688,505 & 11,810 & 227.65 & 0.17 & 0 & 100 & 100 \\ \hline
        \textbf{Respond to CDC} & 122,813 & 21,843 & 5.623 & -0.01 & 4.16 & 34.50 & 6.12 \\ \hline
        \textbf{Verified} & 2,903,733 & 26,428 & 109.87 & 0.10 & 0.10 & 75.61 & -\\ \hline
        \textbf{Respond to verified} & 139,058& 26,205 & 5.31 & -0.01 & 3.96 & 35.07 & 11.02 \\ \hline
        \textbf{Rich media} & 3,032,625 & 99,004 & 30.63 & 0.01 & 11.54 & - & 20.18 \\ \hline
        \textbf{Respond to pictures} & 136,131 & 27,783 & 4.90 & -0.01 & 4.28 & 43.98 & 8.07 \\ \hline
        \textbf{Low credibility} & 36,008 & 17,433 & 2.07 & -0.16 & - & 65.55 & 5.11 \\ \hline
         \textbf{Respond to low credibility} & 702 & 468 & 1.50 & -0.07 & 62.61 & 61.11 & 2.78 \\ \hline
    \end{tabular}
    \label{tab:behavior_echo}
\end{table}

\subsection{Platform affordances, user properties, sentiment and information credibility }\label{sec:twitter_engagement}
We start this section by analyzing how Twitter engagements afforded by the platform like retweets, quote-tweets, likes, mentions, and responses are associated with different themes of COVID discussions. We will specifically focus on direct responses to the CDC and, in turn, direct responses to users from the CDC (as opposed to broadcast messaging). 

\subsubsection{What is in a retweet and what gets more likes?} \label{sec:finding_rt}
As Table \ref{tab:regression_results_1} shows, discussions for or against the vaccine are more likely to be retweeted and to receive likes. While discussions of lock-downs and re-openings, especially in schools (Topics 38 and 65), were less likely to receive likes, they were retweeted at a higher rate. Similarly, engaging in Topic 1, introducing data showing that COVID is not a hoax, increases the chance of being retweeted while reducing the chance of receiving a like.

The chance of receiving likes and being retweeted is higher when Tweets are posted by verified users and when there is a high number of Tweets in the CDC public. Users with a higher follower-following ratio (FFR) and more direct replies are also more likely to receive likes. However, the more direct replies received by a user, the less likely they are to be retweeted. We discuss direct replies next.

\subsubsection{What gets more direct replies and quote-tweets?} \label{findings:replies_quotes}
Engaging in discourse for and against the vaccine (Topic 0) increases the chances of receiving a response and being quote-tweeted. The same applies to discussing masking in schools (Topic 26). Both of these topics were polarizing as they pit people who believed that each mitigation tool was important to control COVID spread and others who were against their implementation because (1) they thought that the mitigation strategies are not as effective as advertised; or (2) they thought that forcing these mitigation measures were against their freedom. A related topic early in the pandemic focused on the very presence of COVID as a virus. While some were questioning the magnitude of the effects on society, others were sharing data, especially from the Johns Hopkins dataset, to counter data from the CDC and other official channels that were considered not forthcoming about the effects of the virus. However, Topic 38, focusing on the effects of lock-downs on society, received fewer responses and quote-tweets. Interestingly, this topic received fewer likes as well. However, it did increase the number of retweets. 

While being verified is more associated with being retweeted, being a verified user makes it less likely to be quote-tweeted. Furthermore, quote-tweeted users have a lower follower-following ratio (influence in the network) and less Tweets in the CDC public. Next, we focus on analyzing direct responses to the CDC.

\paragraph{Responses to the CDC} 
As presented in Table \ref{tab:reply_to_CDC}, the use of rich content was more predictive of responses to the CDC. Much of the rich content included what users referred to as ``receipts,'' screenshots of earlier CDC messages showing the evolving masking guidelines after vaccinations (Topic 4). Other top topics in responses include the vaccines (Topic 0), the role of the CDC in evictions post-COVID, discussing how COVID is airborne (Topic 36), and comparing the response to COVID with the response to the H1N1 breakout under Obama's administration (Topic 56). 

The framing of these responses went in one of three directions: (1) arguing that the CDC's guidelines are not strict enough; (2) arguing that the CDC is introducing mandates without the right to do so; (3) the CDC is overreacting since the effects of COVID are overblown (see Figure \ref{fig:CDC_joke_seatbelt}).

Replies to the CDC were less likely to receive direct replies, likes, retweets, quote-tweets, and usually had lower follower-following ratios.

\paragraph{Direct responses from the CDC}
We found only 58 direct responses from the official CDC  account to 25 accounts based on a question or suggestion. The responses revolved around providing information about the shingles or flu vaccines. A few others were answering questions about the danger of contracting COVID-19 by touching products imported from China. The @CDCgov account answered those accounts by saying there is no danger in handling products from China. 

Now that we analyzed responses to and from the CDC, we will next analyze mention co-occurrence networks along with the @CDCgov account. 

\begin{table}[H]
\centering 
\caption{This Table shows top regression results and the top predictors for Retweets ($\alpha=0.31$, solver=svd) and Likes ($\alpha=0.34$, solver=svd). Table shows significant predictors from regression model. **** p<0.0001; *** p<0.001; ** p<0.01; * p<0.05}
\begin{tabular}{llllll}
\hline
\multicolumn{1}{|c|}{\textbf{Retweets}} & \multicolumn{1}{c|}{\textbf{Ridge}} & \multicolumn{1}{c|}{\textbf{$R^{2}$=0.90}} & \multicolumn{1}{c|}{\textbf{Likes}} & \multicolumn{1}{c|}{\textbf{Ridge}} & \multicolumn{1}{c|}{\textbf{$R^{2}$=0.83}} \\ \hline
\multicolumn{1}{|l|}{\textit{Feature}} & \multicolumn{1}{l|}{\textit{Coefficient}} & \multicolumn{1}{l|}{\textit{p-value}} & \multicolumn{1}{l|}{\textit{Feature}} & \multicolumn{1}{l|}{\textit{Coefficient}} & \multicolumn{1}{l|}{\textit{p-value}} \\ \hline
\multicolumn{1}{|l|}{Topic 0} & \multicolumn{1}{l|}{0.611} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{Topic 0} & \multicolumn{1}{l|}{3.511} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{Topic 1} & \multicolumn{1}{l|}{0.101} & \multicolumn{1}{l|}{*} & \multicolumn{1}{l|}{Topic 1} & \multicolumn{1}{l|}{-0.614} & \multicolumn{1}{l|}{*} \\ \hline
\multicolumn{1}{|l|}{Topic 38} & \multicolumn{1}{l|}{0.072} & \multicolumn{1}{l|}{**} & \multicolumn{1}{l|}{Topic 38} & \multicolumn{1}{l|}{-0.432} & \multicolumn{1}{l|}{**} \\ \hline
\multicolumn{1}{|l|}{Topic 65} & \multicolumn{1}{l|}{0.045} & \multicolumn{1}{l|}{*} & \multicolumn{1}{l|}{Topic 65} & \multicolumn{1}{l|}{-0.23} & \multicolumn{1}{l|}{*} \\ \hline
\multicolumn{1}{|l|}{Verified} & \multicolumn{1}{l|}{2.329} & \multicolumn{1}{l|}{*} & \multicolumn{1}{l|}{Verified} & \multicolumn{1}{l|}{15.033} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{like\_count} & \multicolumn{1}{l|}{2838.533} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{quote\_count} & \multicolumn{1}{l|}{-33146.7} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{quote\_count} & \multicolumn{1}{l|}{7534.939} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{reply\_count} & \multicolumn{1}{l|}{1189.377} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{reply\_count} & \multicolumn{1}{l|}{-1084.07} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{retweet\_count} & \multicolumn{1}{l|}{47676.71} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{count} & \multicolumn{1}{l|}{0.412} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{count} & \multicolumn{1}{l|}{8.882} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{FFR} & \multicolumn{1}{l|}{17.385} & \multicolumn{1}{l|}{*} \\ \hline
\end{tabular}
\label{tab:regression_results_1}
\end{table}

 \begin{table}[ht]
\centering 
\caption{This Table shows top regression results and the top predictors for responses ($\alpha$=0.31, solver=svd) and quote-tweets ($\alpha$=0.68, solver=cholesky), Quotes-tweets, and Responses. Table shows significant predictors from regression model. **** p<0.0001; *** p<0.001; ** p<0.01; * p<0.05}
\begin{tabular}{llllll}
\hline
\multicolumn{1}{|c|}{\textbf{Responses}} & \multicolumn{1}{c|}{\textbf{Ridge }} & \multicolumn{1}{c|}{\textbf{$R^{2}$=0.64}} & \multicolumn{1}{c|}{\textbf{Quote-tweets}} & \multicolumn{1}{c|}{\textbf{Ridge}} & \multicolumn{1}{c|}{\textbf{$R^{2}$=0.70}} \\ \hline
\multicolumn{1}{|l|}{\textit{Feature}} & \multicolumn{1}{l|}{\textit{Coefficient}} & \multicolumn{1}{l|}{\textit{p-value}} & \multicolumn{1}{l|}{\textit{Feature}} & \multicolumn{1}{l|}{\textit{Coefficient}} & \multicolumn{1}{l|}{\textit{p-value}} \\ \hline
\multicolumn{1}{|l|}{Topic 0} & \multicolumn{1}{l|}{0.161} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{Topic 0} & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{Topic 1} & \multicolumn{1}{l|}{-0.06} & \multicolumn{1}{l|}{*} & \multicolumn{1}{l|}{Topic 15} & \multicolumn{1}{l|}{-0.008} & \multicolumn{1}{l|}{**} \\ \hline
\multicolumn{1}{|l|}{Topic 15} & \multicolumn{1}{l|}{0.036} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{Topic 26} & \multicolumn{1}{l|}{0.011} & \multicolumn{1}{l|}{*} \\ \hline
\multicolumn{1}{|l|}{Topic 26} & \multicolumn{1}{l|}{0.004} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{Topic 38} & \multicolumn{1}{l|}{-0.005} & \multicolumn{1}{l|}{*} \\ \hline
\multicolumn{1}{|l|}{Topic 38} & \multicolumn{1}{l|}{-0.001} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{Verified} & \multicolumn{1}{l|}{-0.032} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{Verified} & \multicolumn{1}{l|}{0.732} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{reply\_count} & \multicolumn{1}{l|}{856.81} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{like\_count} & \multicolumn{1}{l|}{32.959} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{retweet\_count} & \multicolumn{1}{l|}{962.706} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{quote\_count} & \multicolumn{1}{l|}{2964.705} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{count} & \multicolumn{1}{l|}{-1.813} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{retweet\_count} & \multicolumn{1}{l|}{-504.582} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{FFR} & \multicolumn{1}{l|}{-0.666} & \multicolumn{1}{l|}{****} \\ \hline
\multicolumn{1}{|l|}{count} & \multicolumn{1}{l|}{10.537} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{FFR} & \multicolumn{1}{l|}{2.828} & \multicolumn{1}{l|}{****} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
\label{tab:regression_results_2}
\end{table}

\begin{table}[ht]
\caption{Predictors for direct replies to the CDC. The table shows the average metrics from RandomSearch and the hyperparameters for the top model. They also show the top positive and negative predictors as determined using SHAP.}
\centering
\small
\begin{tabular}{|c||c|}
    \hline
    & \textbf{Reply to CDC} \\
    \hline
    \textbf{Average Metrics} & \\
    Accuracy & 0.645 \\
    Precision & 0.626 \\
    Recall & 0.767 \\
    F1 & 0.684 \\
    AUC & 0.716 \\
    \hline
    \textbf{Top Model (GBC)} &  est=150, max. depth=5, learning rate=0.3\\
    Accuracy & 0.752 \\
    Precision & 0.725 \\
    Recall & 0.811 \\
    F1 & 0.766 \\
    AUC & 0.837 \\
    \hline
    \textbf{Positive Features} & 0, 4, 27, 36,56, Rich \\
    \textbf{Negative Features} & Rep, Like, FFR, RT, 7, 15, 15, 61, QT, 29, 9, 19, 8, 56 \\
    \hline
\end{tabular}
\label{tab:reply_to_CDC}
\end{table}

\begin{table}[ht]
  \caption{Part 1 of Classifiers: Performance metrics for Positive, Neutral, Negative, and Reply to CDC classifiers. The table shows the average metrics from RandomSearch and the hyperparameters for the top model. They also show the top positive and negative predictors as determined using SHAP.}
    \centering
    \small
    \begin{tabular}{|l||p{2.5cm}|p{2.5cm}|p{2.5cm}|}
        \hline
        & \textbf{Positive} & \textbf{Neutral} & \textbf{Negative} \\
        \hline
        \textbf{Average Metrics} & & & \\
        Accuracy & 0.668 & 0.681 & 0.688 \\
        Precision & 0.667 & 0.684 & 0.715 \\
        Recall & 0.717 & 0.713 & 0.593 \\
        F1 & 0.685 & 0.689 & 0.633 \\
        AUC & 0.700 & 0.719 & 0.727 \\
        \hline
        \textbf{Top Model (RF)} & est=50; mins=5, max=None & est=100; mins=5, max=10 & est=100; mins=5, max=10 \\
        Accuracy & 0.984 & 0.983 & 0.985 \\
        Precision & 0.985 & 0.983 & 0.984 \\
        Recall & 0.982 & 0.983 & 0.985 \\
        F1 & 0.984 & 0.983 & 0.985 \\
        AUC & 0.999 & 0.998 & 0.999 \\
        \hline
        \textbf{Positive Features} & RT, 15, QT, FFR, VR, 1 & 5, FFR, 21, 14, 9, 32, 63 & 19, 25 \\
        \textbf{Negative Features} & 25, Rep, 16, 2, 54, 23, 8, 14, 44,29,56  & 70, Rep, QT, Like & FFR, 14, 30, RT, 21 \\
        \hline
    \end{tabular}
\label{tab:classifier_metrics_part1}
\end{table}



\begin{table}[ht]
  \caption{Part 2 of Classifiers: Performance metrics for Photo, Low Quality, and Verified classifiers. The table shows the average metrics from RandomSearch and the hyperparameters for the top model. They also show the top positive and negative predictors as determined using SHAP.}
    \centering
    \small
    \begin{tabular}{|l||p{2.5cm}|p{2.5cm}|p{2.5cm}|}
        \hline
        & \textbf{Rich Media} & \textbf{Low Credibility} & \textbf{Verified} \\
        \hline
        \textbf{Average Metrics} & & & \\
        Accuracy & 0.719 & 0.699 & 0.830 \\
        Precision & 0.820 & 0.708 & 0.838 \\
        Recall & 0.529 & 0.754 & 0.812 \\
        F1 & 0.619 & 0.718 & 0.822 \\
        AUC & 0.756 & 0.789 & 0.905 \\
        \hline
        \textbf{Top Model (RF)} & est=100; mins=5, max=10 & est=100; min=2, max=None & est=100; mins=5, max=10\\
        Accuracy & 0.996 & 0.782 & 0.894 \\
        Precision & 0.998 & 0.803 & 0.876 \\
        Recall & 0.994 & 0.748 & 0.916 \\
        F1 & 0.996 & 0.775 & 0.896 \\
        AUC & 0.995 & 0.872 & 0.964 \\
        \hline
        \textbf{Positive Features} & RT, FFR, QT, Like, Rep, 5 & 19, Rich, 7, VR & FFR, QT, RT, Like, Rep, 14, Rich \\
        \textbf{Negative Features} & VR, 6, 16, 61 & Like, Rep, RT, 23, 32 & Count, 21 \\
        \hline
    \end{tabular}
\label{tab:classifier_metrics_part2}
\end{table}

\subsubsection{What is in a mention?} \label{sec:finding_mention}
Mentioning accounts can be directing a message to an account expecting a response or increasing attention to the message by mentioning an influential account in the network, in this case, the CDC. The co-occurrence mentions network \cite{Nasim_2017} shown in Figure \ref{fig:mention_cooccurence} where the top accounts mentioned alongside the @CDCGov account are presented in the following groups:
\begin{enumerate}
    \item Pharmaceutical companies like @pfizer (specifically focused on the vaccine production)
    \item Public health professionals/academics: @DrEricDing (see \S\ref{related:verified_acct})
    \item Politicians: @VP, @secazar, @joebiden, @govrondesantis, @mikepense, @presssec, @kamalaharris, @statedepartment, @nycgovcuomo,@joebiden, @gop, @statedept, @cdcdirector
    \item News corporations and journalists: @foxnews, @jaketapper, @cnn, @abc, @cbsnews, @nbcnews @msnbc, @maddow, @alexberenson (this last account is a verified journalist who happens to share low-credibility information sources; more in \S\ref{sec:verified_accts})
    \item State and federal agencies: @fema (Federal Emergency Management Agency), @nih, @us\_fda (US Food and Drug Administration), @dhsgov (Department of Homeland Security), @hhsgov (health and human services), @cdcmmwr (Morbidity and Mortality Weekly Report), @drnancym\_cdc, @HealthyFla (Florida Dept. of Health; see \S\ref{sec:covid_test})
\end{enumerate}


The results of our ERGM model, which analyzes the likelihood of a mention tie, are summarized in Table \ref{tab:ERGM}. Our edges (intercept) parameter is negative and significant. This means that there is a high `cost' to the creation of a tie in the network \cite{keegan_et_al_2012}[p.432]. In our sparse network, we found a positive ``mutual''parameter suggesting a higher likelihood of tie creation associated with reciprocation. In other words, when one user mentions another, they are more likely to mention the original user. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{mentionsnetworksCDC.png}
    \caption{Mention co-occurrence network showing top accounts mentioned along with the CDC account.}
    \label{fig:mention_cooccurence}
\end{figure}

When analyzing node characteristics, we found that most of the discussion themes identified in \S\ref{sec:topics} decreased the likelihood of creating a mention tie. The only theme that increased the likelihood of the creation of a mention tie was the one focused on non-COVID discourse probably due to the high connectivity between those working with opioid addiction patients, pain activists, and veterans (discussed in more detail in \S\ref{sec:cdc_non_covid})). We found that out-degree tie formation was more likely for users who posted more using less credible sources. In other words, users who relied on less reputable sources were more likely to mention others while they themselves were less likely to be mentioned. Both negative and positive sentiment decreased the likelihood of the creation of mention ties, while neutral sentiment increased the likelihood. The more the use of rich media in Tweets, the less likely the creation of mention ties. Finally, verified users are less likely to have mention ties with other users. 

\begin{table}[ht]
\caption{Exponential family random graph model of mentions network. A smaller value means the likelihood of creating a mention tie is smaller and vice-versa. **** p<0.0001; *** p<0.001; ** p<0.01; * p<0.05}
\begin{tabular}{|l|r|r|r|l|}

\hline
                                & \multicolumn{1}{l|}{Estimate} & \multicolumn{1}{l|}{Std. Error} & \multicolumn{1}{l|}{z value} &     \\ \hline
nodeocov.verified               & -0.062                        & 0.012                           & -4.979                       & *** \\ \hline
nodeicov.verified               & -0.205                        & 0.013                           & -15.236                      & ** \\ \hline
nodematch.top\_theme.Mitigation & -0.147                        & 0.007                           & -20.031                      & *** \\ \hline
nodematch.top\_theme.Non-COVID  & 1.236                         & 0.032                           & 38.792                       & *** \\ \hline
nodematch.top\_theme.Politics   & -0.205                        & 0.011                           & -18.738                      & *** \\ \hline
nodematch.top\_theme.Test       & -0.267                        & 0.022                           & -12.250                      & ** \\ \hline
nodeocov.lowq-credibility             & 0.096                         & 0.024                           & 3.948                        & *** \\ \hline
nodeicov.lowq-credibility             & -0.231                        & 0.029                           & -7.980                       & *** \\ \hline
nodeicov.photo                  & -0.267                        & 0.008                           & -32.107                      & *** \\ \hline
nodematch.sentiment.negative    & -0.237                        & 0.009                           & -25.842                      & *** \\ \hline
nodematch.sentiment.neutral     & 0.381                         & 0.011                           & 33.583                       & *** \\ \hline
nodematch.sentiment.positive    & -0.078                        & 0.008                           & -9.781                       & *** \\ \hline
edges                           & -8.896                        & 0.004                           & -2000.335                    & *** \\ \hline
mutual                          & 3.483                         & 0.063                           & 55.150                       & *** \\ \hline
\end{tabular}
    \label{tab:ERGM}
\end{table}


\subsection{Sentiment, rich media, and low credibility sources} \label{sec:sent_photo_credibility}
In this section, we will analyze the qualities of positive, neutral, and negative labeled Tweets, as well as ones labeled with the use of rich media (e.g., images) and low-credibility sources. 

\subsubsection{Positive Tweets} \label{subsec:positive}
A higher retweet and quote Tweet count, being verified, and having a higher follower-following ratio are all more positively predictive of positive Tweets. Sharing data sources pointing to the seriousness of COVID (Topic 1), but also to good news about dropping rates of infection (Topic 15).

Positive Tweets are less likely to receive direct responses. They are also less likely to discuss COVID and seasonal flu infection and mortality rates (Topics 16 \& 25), the efficacy of masks (Topics 2 and 54), or calling for obedience to the CDC mitigation guidelines in general (Topic 44). They tend to make less mention of political discourse like Trump's CDC (Topic 8), the political/legislative response to COVID (Topic 29), or comparing the COVID response to H1N1 response under Obama's administration (Topic 56).  

\subsubsection{Neutral Tweets} \label{subsec:neutral}
Higher follower-following ratio increases the chance of a neutral Tweet. Neutral tweets tend to receive fewer responses, quote-tweets, and likes. 

Sports players and attendance guidelines (Topic 21) and social distancing guidelines (six feet apart; Topic 63) are also positively associated with neutral Tweets. These are often posts by users with high FFR, usually at a local level, like high school and college athletic departments, coaches, and sports commentators who, while not verified, have large followings. Many of the posts simply stated the current requirements for attending sports events (e.g., in-door masking for intramural sports or social distancing requirements). 

The lack of clarity in CDC guidelines (Topic 9), the attack and defense of the CDC (Topic 14), and the administrative and legislative response to COVID (Topic 32) are positively predictive of neutral Tweets. While defending/attacking the CDC might sound polarizing, the Tweets themselves can have a more neutral sentiment since they can be nuanced. For example, the author of the Tweet could specify that while they support the CDC's efforts, they do not think the organization is doing enough to counter the virus. Specifically, they could focus on the fact that the CDC only publishes data when it can have a more positive context – when the COVID infection numbers are decreasing. For reference, Table \ref{tab:behavior_echo} shows that CDC Tweets are more positive than any other entity, cluster, or theme with an average VADER score of 0.17. 

\subsubsection{Negative Tweets} \label{subsec:negative}
Higher retweets and follower-following ratios are less predictive of negative Tweets. The more a Tweet discusses COVID infections and mortality rates (Topic 25) or the opioid pandemic data (Topic 19), the more they are likely to evince a negative sentiment. The first topic can be more negative because it usually focuses on attacking the CDC for reporting mortality numbers that are unexpectedly high or low (note that while COVID infection numbers are heavily discussed in positive Tweets, positive Tweets do not focus on mortality rates). Negative tweets  are also less focused on attacking/defending the CDC (Topic 14) and in-person gathering guidelines. 

\subsubsection{Tweets using rich media} \label{subsec:rich_Tweets}
Tweets using rich media are more likely to be retweeted, liked, quote-tweeted, get a reply, and engage with the CDC (Topic 5). Tweets using rich media are less likely to be posted from verified accounts, or to discuss lack of up-to-date COVID testing data (Topic 6), seasonal flu mortality rates (Topic 16) or music and stress (Topic 61).

\subsubsection{Tweets using low credibility sources} \label{subsec:low_credibility}
The use of rich media and verified accounts are more predictive of the use of low credibility sources. The focus on discussing the opioid pandemic (Topic 19) and COVID mortality rates (Topic 7) are also positively predictive of low credibility sources. 

Tweets using low credibility sources are less likely to be liked, retweeted, get responses, or engage in discussions regarding legislative and administrative responses to COVID (Topic 32) or Salmonella outbreaks (Topic 23).

\subsection{Verified accounts and accounts with high follower-following ratios} \label{sec:verified_accts}
Verified accounts are more likely to be retweeted, quote-tweeted, liked, get direct responses, use rich media and engage in attacking or defending the CDC (Topic 14). Verified accounts are less likely to Tweet in the CDC public (Tweet count) and less likely to discuss Sports players and attendance guidelines (Topic 21). While verified accounts engaged with less Tweets than other users, their messages were retweeted at a higher rate which is in-line with the high echo value for verified accounts indicated in Table \ref{tab:behavior_echo}. It is also interesting to note that responses to verified accounts in general, and the CDC in particular were around 5, which means that the user received 5 retweets for an engagement with a verified account or the CDC. 

While the use of low-credibility sources is not predictive of verified accounts, verified accounts are predictive of the use of low credibility sources in a Tweet. In other words, some verified accounts used low credibility sources in their engagement. One example is @alexberenson, a journalist who pushed back against most of the CDC's mitigation strategies. Berenson, with a verified journalist account, used several low-credibility sources and was mentioned along with the @CDCGov account with high frequency (see \S\ref{sec:finding_mention}) which would expand his audience further.

Accounts with high FFR were more likely to receive likes and responses. They were more likely to engage in positive or neutral messaging and use rich media in their Tweets.


==> method3.tex <==
\section{Study3:Methods}



